Contrastive Gradient Guidance for Test-Time Multi-Preference Alignment of Diffusion Models

Aligning pre-trained diffusion models with multiple context-dependent preferences requires adapting generation at test time rather than relying on offline fine-tuning, which requires hyperparameter tuning and a new training run for each preference trade-off. Existing approaches compress diverse preferences into a single scalar reward objective for fine-tuning or test-time guidance rather than directly reusing existing generative experts released for different purposes and obtained through different fine-tuning methods. In this work, we propose Contrastive Gradient Guidance (CGG), a test-time compositional generative framework that reformulates multi-preference alignment as a composition of distributions. CGG represents each preference as a contrastive preference pair of favored experts and unfavored anti-experts, whose score difference forms a contrastive gradient guidance signal that combines denoising directions (gradients) from off-the-shelf diffusion models during sampling. Experiments show that CGG reuses pre-trained and fine-tuned models as favored experts or anti-experts to control output style and safety, and that it can be combined with existing sampling-based reward guidance. With a single fixed scale per pair, CGG composes five preferences at once and gives a more balanced trade-off across text-image preference, concept control, photographic fidelity, and safety than offline fine-tuning, weight-space merging, and reward steering.

==> Makefile <==
# One-step build for the arXiv version (single-column gvcmix style).
# Does not touch the AAAI sources in ../ .
#
#   make             build main.pdf (pdflatex + bibtex, rerun until refs settle)
#   make open        build, then open main.pdf
#   make check       pages / size / undefined references
#   make arxiv       pack arxiv_submission.tar.gz (includes main.bbl)
#   make clean       remove LaTeX intermediates (keeps main.pdf and main.bbl)
#   make distclean   also remove main.pdf, main.bbl and the tarball

.PHONY: all pdf open check arxiv clean distclean FORCE

LATEXMK       ?= latexmk
LATEXMK_FLAGS ?= -pdf -interaction=nonstopmode -halt-on-error -file-line-error
OPEN          ?= open

all: main.pdf

pdf: main.pdf

# latexmk records every input it reads (sections/, tables/, figures/, main.bib,
# gvcmix.cls, ...) and reruns pdflatex/bibtex only as needed, so always hand
# control to it; it returns immediately when nothing has changed.
main.pdf: FORCE
	$(LATEXMK) $(LATEXMK_FLAGS) main.tex

open: main.pdf
	$(OPEN) main.pdf

check: main.pdf
	@printf "pages: " && pdfinfo main.pdf | awk '/^Pages:/{print $$2}'
	@printf "size:  " && (stat -f '%z bytes' main.pdf 2>/dev/null || stat -c '%s bytes' main.pdf)
	@grep -E 'undefined (references|citations)|multiply-defined' main.log || echo "no undefined/multiply-defined labels"

# Source bundle for arXiv upload.  arXiv does not run bibtex, so main.bbl
# must be included; build artefacts and the compiled PDF are excluded.
# The two Ghibli figures are included as PNG; their PDF originals (28 MB) are
# excluded from the bundle in case they are still lying around in figures/.
arxiv: main.pdf
	rm -f arxiv_submission.tar.gz
	tar czf arxiv_submission.tar.gz \
	    --exclude='figures/style_avoidance_ghibli.pdf' \
	    --exclude='figures/style_avoidance_ghibli_full.pdf' \
	    --exclude='figures/.DS_Store' --exclude='figures/*/.DS_Store' \
	    00README.json main.tex main.bbl main.bib gvcmix.cls natbib.sty \
	    sections tables figures
	@ls -lh arxiv_submission.tar.gz
	@echo "NOTE: arXiv's default upload limit is 50 MB; see README.md if the bundle is larger."

clean:
	rm -f *.aux *.blg *.log *.out *.toc *.fls *.fdb_latexmk *.synctex.gz

distclean: clean
	rm -f main.bbl main.pdf arxiv_submission.tar.gz

FORCE:

